Calibrating Panoramic Depth Estimation for Practical Localization and Mapping

The absolute depth values of surrounding environments provide crucial cues for various assistive technologies, such as localization, navigation, and 3D structure estimation. We propose that accurate depth estimated from panoramic images can serve as a powerful and light-weight input for a wide range of downstream tasks requiring 3D information. While panoramic images can easily capture the surrounding context from commodity devices, the estimated depth shares the limitations of conventional image-based depth estimation; the performance deteriorates under large domain shifts and the absolute values are still ambiguous to infer from 2D observations. By taking advantage of the holistic view, we mitigate such effects in a self-supervised way and fine-tune the network with geometric consistency during the test phase. Specifically, we construct a 3D point cloud from the current depth prediction and project the point cloud at various viewpoints or apply stretches on the current input image to generate synthetic panoramas. Then we minimize the discrepancy of the 3D structure estimated from synthetic images without collecting additional data. We empirically evaluate our method in robot navigation and map-free localization where our method shows large performance enhancements. Our calibration method can therefore widen the applicability under various external conditions, serving as a key component for practical panorama-based machine vision systems. Code is available through the following link: \url{https://github.com/82magnolia/panoramic-depth-calibration}.

==> tables/supp_full_aggregated.tex <==
\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.4460 & 0.2163 & 0.1705 & 0.6222 & 0.1053 & 0.6960 & 0.9412 & 0.9801 \\
Schneider et al.~\cite{batchnorm_update} & 0.5226 & 0.2296 & 0.2340 & 0.7984 & 0.1254 & 0.6334 & 0.9006 & 0.9599 \\
Tent~\cite{tent} & 0.4418 & 0.2143 & 0.1684 & 0.6173 & 0.1046 & 0.7028 & 0.9416 & 0.9803 \\
Flip Consistency & 0.4349 & 0.2104 & 0.1625 & 0.6132 & 0.1028 & 0.7035 & 0.9417 & 0.9804 \\
Mask Consistency & 0.4153 & 0.2005 & 0.1513 & 0.5910 & 0.0996 & 0.7361 & 0.9437 & 0.9811 \\
Photometric Consistency & 0.4467 & 0.2187 & 0.1703 & 0.6222 & 0.1055 & 0.6861 & 0.9425 & 0.9807 \\
Pseudo Labelling & 0.4235 & 0.2068 & 0.1558 & 0.5923 & 0.1012 & 0.7157 & 0.9445 & 0.9819 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.4267 & 0.2018 & 0.1567 & 0.6208 & 0.1021 & 0.7320 & 0.9390 & 0.9792 \\
CrDoCo~\cite{chen2019crdoco} & 0.4229 & 0.2041 & 0.1531 & 0.5987 & 0.1012 & 0.7266 & 0.9424 & 0.9810 \\
Feature Consistency & 0.4237 & 0.1996 & 0.1533 & 0.6158 & 0.1013 & 0.7359 & 0.9400 & 0.9795 \\
Ground-Truth Training & 0.3490 & 0.1725 & 0.1196 & 0.5180 & 0.0895 & 0.7965 & 0.9565 & 0.9854 \\
Ours & 0.3653 & 0.1798 & 0.1297 & 0.5253 & 0.0921 & 0.7910 & 0.9512 & 0.9834 \\
\bottomrule
\end{tabularx}
}
\caption{Full aggregated results for offline adaptation using 5\% of the panorama images for training}
\end{table*}

    \smallskip

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.4443 & 0.2157 & 0.1699 & 0.6232 & 0.1054 & 0.6973 & 0.9422 & 0.9802 \\
Schneider et al.~\cite{batchnorm_update} & 0.5186 & 0.2280 & 0.2302 & 0.7932 & 0.1241 & 0.6336 & 0.9037 & 0.9614 \\
Tent~\cite{tent} & 0.4399 & 0.2136 & 0.1676 & 0.6183 & 0.1046 & 0.7052 & 0.9428 & 0.9803 \\
Flip Consistency & 0.4223 & 0.2057 & 0.1564 & 0.5987 & 0.1013 & 0.7174 & 0.9435 & 0.9809 \\
Mask Consistency & 0.4190 & 0.2018 & 0.1539 & 0.5994 & 0.1009 & 0.7345 & 0.9426 & 0.9804 \\
Photometric Consistency & 0.4394 & 0.2149 & 0.1667 & 0.6123 & 0.1043 & 0.6978 & 0.9440 & 0.9810 \\
Pseudo Labelling & 0.4296 & 0.2076 & 0.1588 & 0.6107 & 0.1027 & 0.7149 & 0.9431 & 0.9807 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.4294 & 0.2027 & 0.1588 & 0.6290 & 0.1030 & 0.7307 & 0.9377 & 0.9785 \\
CrDoCo~\cite{chen2019crdoco} & 0.4239 & 0.2045 & 0.1548 & 0.6045 & 0.1018 & 0.7268 & 0.9420 & 0.9806 \\
Feature Consistency & 0.4277 & 0.2005 & 0.1578 & 0.6291 & 0.1028 & 0.7345 & 0.9373 & 0.9781 \\
Ground-Truth Training & 0.3398 & 0.1703 & 0.1167 & 0.5019 & 0.0882 & 0.8039 & 0.9580 & 0.9857 \\
Ours & 0.3620 & 0.1784 & 0.1291 & 0.5231 & 0.0920 & 0.7951 & 0.9511 & 0.9830 \\
\bottomrule
\end{tabularx}
}
\caption{Full aggregated results for offline adaptation using 10\% of the panorama images for training}
\end{table*}

    \smallskip

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.4412 & 0.2143 & 0.1675 & 0.6211 & 0.1053 & 0.7012 & 0.9424 & 0.9804 \\
Schneider et al.~\cite{batchnorm_update} & 0.4178 & 0.1859 & 0.1593 & 0.7212 & 0.1077 & 0.7427 & 0.9403 & 0.9789 \\
Tent~\cite{tent} & 0.4274 & 0.2044 & 0.1582 & 0.6457 & 0.1052 & 0.7329 & 0.9437 & 0.9805 \\
Flip Consistency & 0.4414 & 0.2037 & 0.1594 & 0.7375 & 0.1092 & 0.7115 & 0.9314 & 0.9745 \\
Mask Consistency & 0.4601 & 0.2170 & 0.1679 & 0.7523 & 0.1130 & 0.6652 & 0.9258 & 0.9723 \\
Photometric Consistency & 0.4595 & 0.2354 & 0.1735 & 0.6633 & 0.1120 & 0.6254 & 0.9355 & 0.9807 \\
Pseudo Labelling & 0.4344 & 0.2143 & 0.1537 & 0.6812 & 0.1085 & 0.6824 & 0.9358 & 0.9774 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.4022 & 0.1984 & 0.1421 & 0.6303 & 0.1024 & 0.7471 & 0.9408 & 0.9791 \\
CrDoCo~\cite{chen2019crdoco} & 0.4646 & 0.2191 & 0.1727 & 0.7665 & 0.1139 & 0.6663 & 0.9245 & 0.9708 \\
Feature Consistency & 0.6412 & 0.2511 & 0.3080 & 1.1059 & 0.1683 & 0.5686 & 0.8090 & 0.9028 \\
Ground-Truth Training & 0.2388 & 0.1110 & 0.0736 & 0.4351 & 0.0713 & 0.8846 & 0.9719 & 0.9903 \\
Ours & 0.3234 & 0.1494 & 0.1045 & 0.5246 & 0.0865 & 0.8300 & 0.9607 & 0.9872
 \\
\bottomrule
\end{tabularx}
}
\caption{Full aggregated results for online adaptation in dataset shift}
\end{table*}

    \smallskip

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.3862 & 0.2185 & 0.1480 & 0.5135 & 0.1039 & 0.6848 & 0.9516 & 0.9836 \\
Schneider et al.~\cite{batchnorm_update} & 0.4075 & 0.2255 & 0.1597 & 0.5643 & 0.1035 & 0.6778 & 0.9505 & 0.9852 \\
Tent~\cite{tent} & 0.3653 & 0.2072 & 0.1349 & 0.5011 & 0.1022 & 0.7276 & 0.9542 & 0.9843 \\
Flip Consistency & 0.3040 & 0.1864 & 0.0978 & 0.4087 & 0.0942 & 0.7753 & 0.9591 & 0.9867 \\
Mask Consistency & 0.3246 & 0.2053 & 0.1057 & 0.4231 & 0.1001 & 0.7121 & 0.9537 & 0.9861 \\
Photometric Consistency & 0.3634 & 0.2132 & 0.1325 & 0.4840 & 0.1054 & 0.6909 & 0.9510 & 0.9828 \\
Pseudo Labelling & 0.3564 & 0.2219 & 0.1235 & 0.4543 & 0.1041 & 0.6781 & 0.9509 & 0.9855 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.3433 & 0.2215 & 0.1213 & 0.4334 & 0.1045 & 0.6962 & 0.9484 & 0.9844 \\
CrDoCo~\cite{chen2019crdoco} & 0.3347 & 0.2081 & 0.1090 & 0.4445 & 0.1022 & 0.7055 & 0.9504 & 0.9853 \\
Feature Consistency & 0.4775 & 0.2459 & 0.2082 & 0.7111 & 0.1480 & 0.5827 & 0.8413 & 0.9292 \\
Ground-Truth Training & 0.1912 & 0.1125 & 0.0545 & 0.2984 & 0.0695 & 0.8855 & 0.9724 & 0.9911 \\
Ours & 0.2362 & 0.1333 & 0.0690 & 0.3605 & 0.0779 & 0.8584 & 0.9692 & 0.9894 \\
\bottomrule
\end{tabularx}
}
\caption{Full aggregated results for online adaptation in low lighting}
\end{table*}

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.4141 & 0.2325 & 0.1615 & 0.5441 & 0.1110 & 0.6454 & 0.9404 & 0.9781 \\
Schneider et al.~\cite{batchnorm_update} & 0.4089 & 0.2256 & 0.1588 & 0.5636 & 0.1034 & 0.6742 & 0.9511 & 0.9857 \\
Tent~\cite{tent} & 0.3926 & 0.2207 & 0.1481 & 0.5342 & 0.1100 & 0.6901 & 0.9433 & 0.9788 \\
Flip Consistency & 0.3216 & 0.1904 & 0.1041 & 0.4472 & 0.1003 & 0.7608 & 0.9481 & 0.9807 \\
Mask Consistency & 0.3378 & 0.2118 & 0.1109 & 0.4395 & 0.1024 & 0.6995 & 0.9504 & 0.9853 \\
Photometric Consistency & 0.4190 & 0.2492 & 0.1597 & 0.5321 & 0.1153 & 0.5810 & 0.9396 & 0.9804 \\
Pseudo Labelling & 0.3673 & 0.2295 & 0.1281 & 0.4615 & 0.1069 & 0.6636 & 0.9456 & 0.9840 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.3592 & 0.2263 & 0.1262 & 0.4514 & 0.1057 & 0.6888 & 0.9478 & 0.9844 \\
CrDoCo~\cite{chen2019crdoco} & 0.3379 & 0.2125 & 0.1105 & 0.4394 & 0.1026 & 0.7026 & 0.9504 & 0.9856 \\
Feature Consistency & 0.4901 & 0.2495 & 0.2149 & 0.7294 & 0.1538 & 0.5703 & 0.8295 & 0.9242 \\
Ground-Truth Training & 0.1916 & 0.1126 & 0.0541 & 0.3003 & 0.0698 & 0.8855 & 0.9720 & 0.9908 \\
Ours & 0.2527 & 0.1393 & 0.0749 & 0.3892 & 0.0834 & 0.8437 & 0.9627 & 0.9860
 \\
\bottomrule
\end{tabularx}
}
\caption{Full aggregated results for online adaptation in white balance change}
\end{table*}

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.4048 & 0.2312 & 0.1565 & 0.5245 & 0.1048 & 0.6817 & 0.9489 & 0.9841 \\
Schneider et al.~\cite{batchnorm_update} & 0.4062 & 0.2242 & 0.1552 & 0.5587 & 0.1027 & 0.6768 & 0.9522 & 0.9861 \\
Tent~\cite{tent} & 0.3792 & 0.2173 & 0.1413 & 0.5046 & 0.1022 & 0.7266 & 0.9524 & 0.9851 \\
Flip Consistency & 0.3292 & 0.2072 & 0.1089 & 0.4191 & 0.0983 & 0.7360 & 0.9560 & 0.9868 \\
Mask Consistency & 0.3341 & 0.2121 & 0.1079 & 0.4271 & 0.1008 & 0.6975 & 0.9549 & 0.9870 \\
Photometric Consistency & 0.4192 & 0.2597 & 0.1717 & 0.5157 & 0.1144 & 0.5920 & 0.9373 & 0.9816 \\
Pseudo Labelling & 0.3506 & 0.2202 & 0.1187 & 0.4383 & 0.1018 & 0.7043 & 0.9530 & 0.9863 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.3338 & 0.2138 & 0.1157 & 0.4229 & 0.1007 & 0.7275 & 0.9518 & 0.9852 \\
CrDoCo~\cite{chen2019crdoco} & 0.3284 & 0.2096 & 0.1079 & 0.4246 & 0.1000 & 0.7255 & 0.9527 & 0.9862 \\
Feature Consistency & 0.3985 & 0.2103 & 0.1518 & 0.5914 & 0.1230 & 0.6646 & 0.8945 & 0.9620 \\
Ground-Truth Training & 0.1830 & 0.1076 & 0.0520 & 0.2904 & 0.0672 & 0.8962 & 0.9742 & 0.9915 \\
Ours & 0.2332 & 0.1308 & 0.0672 & 0.3599 & 0.0766 & 0.8666 & 0.9705 & 0.9898
 \\
\bottomrule
\end{tabularx}
}
\caption{Full aggregated results for online adaptation in image gamma change}
\end{table*}

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.4950 & 0.1892 & 0.1829 & 0.7659 & 0.1054 & 0.7289 & 0.9341 & 0.9751 \\
Schneider et al.~\cite{batchnorm_update} & 0.6117 & 0.2002 & 0.2547 & 1.0768 & 0.1429 & 0.6604 & 0.8783 & 0.9495 \\
Tent~\cite{tent} & 0.5021 & 0.1887 & 0.1845 & 0.8251 & 0.1093 & 0.7296 & 0.9321 & 0.9745 \\
Flip Consistency & 0.5491 & 0.1913 & 0.2019 & 0.9298 & 0.1123 & 0.7160 & 0.9180 & 0.9677 \\
Mask Consistency & 0.5451 & 0.1922 & 0.1971 & 0.9296 & 0.1100 & 0.7177 & 0.9200 & 0.9710 \\
Photometric Consistency & 0.5097 & 0.1936 & 0.1844 & 0.8308 & 0.1097 & 0.6993 & 0.9344 & 0.9761 \\
Pseudo Labelling & 0.5160 & 0.1876 & 0.1810 & 0.8770 & 0.1071 & 0.7269 & 0.9279 & 0.9751 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.5268 & 0.1843 & 0.1874 & 0.9118 & 0.1076 & 0.7399 & 0.9241 & 0.9720 \\
CrDoCo~\cite{chen2019crdoco} & 0.5554 & 0.1905 & 0.2032 & 0.9755 & 0.1111 & 0.7230 & 0.9164 & 0.9680 \\
Feature Consistency & 0.7215 & 0.2214 & 0.3261 & 1.2991 & 0.1578 & 0.6197 & 0.8368 & 0.9197 \\
Ground-Truth Training & 0.3437 & 0.1320 & 0.1135 & 0.6072 & 0.0804 & 0.8599 & 0.9665 & 0.9879 \\
Ours & 0.4239 & 0.1591 & 0.1430 & 0.6977 & 0.0931 & 0.8032 & 0.9525 & 0.9844
 \\
\bottomrule
\end{tabularx}
}
\caption{Full aggregated results for online adaptation in large scenes}
\end{table*}

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.3116 & 0.1770 & 0.0975 & 0.4292 & 0.0887 & 0.7878 & 0.9573 & 0.9872 \\
Schneider et al.~\cite{batchnorm_update} & 0.4010 & 0.2347 & 0.1911 & 0.5508 & 0.1021 & 0.6841 & 0.9103 & 0.9768 \\
Tent~\cite{tent} & 0.3071 & 0.1743 & 0.0953 & 0.4282 & 0.0889 & 0.7938 & 0.9577 & 0.9873 \\
Flip Consistency & 0.3049 & 0.1772 & 0.0899 & 0.4105 & 0.0890 & 0.7847 & 0.9618 & 0.9879 \\
Mask Consistency & 0.2724 & 0.1646 & 0.0781 & 0.3666 & 0.0835 & 0.8059 & 0.9657 & 0.9894 \\
Photometric Consistency & 0.2900 & 0.1700 & 0.0904 & 0.3995 & 0.0858 & 0.7962 & 0.9584 & 0.9877 \\
Pseudo Labelling & 0.3000 & 0.1764 & 0.0906 & 0.4033 & 0.0864 & 0.7907 & 0.9623 & 0.9889 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.2743 & 0.1674 & 0.0806 & 0.3674 & 0.0843 & 0.7996 & 0.9643 & 0.9890 \\
CrDoCo~\cite{chen2019crdoco} & 0.2629 & 0.1598 & 0.0741 & 0.3576 & 0.0826 & 0.8121 & 0.9643 & 0.9885 \\
Feature Consistency & 0.2881 & 0.1606 & 0.0831 & 0.4089 & 0.0902 & 0.7829 & 0.9541 & 0.9836 \\
Ground-Truth Training & 0.2168 & 0.1299 & 0.0592 & 0.3122 & 0.0725 & 0.8575 & 0.9688 & 0.9897 \\
Ours & 0.2440 & 0.1420 & 0.0674 & 0.3498 & 0.0780 & 0.8351 & 0.9657 & 0.9888
 \\
\bottomrule
\end{tabularx}
}
\caption{Full aggregated results for online adaptation in small scenes}
\end{table*}


\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.5254 & 0.3275 & 0.3367 & 0.7433 & 0.1611 & 0.5327 & 0.8073 & 0.9163 \\
Schneider et al.~\cite{batchnorm_update} & 0.5562 & 0.3355 & 0.3704 & 0.7965 & 0.1669 & 0.4781 & 0.7927 & 0.9177 \\
Tent~\cite{tent} & 0.5076 & 0.3133 & 0.3088 & 0.7228 & 0.1585 & 0.5461 & 0.8163 & 0.9216 \\
Flip Consistency & 0.4524 & 0.2730 & 0.2106 & 0.6588 & 0.1417 & 0.5770 & 0.8534 & 0.9439 \\
Mask Consistency & 0.4701 & 0.2777 & 0.2259 & 0.6998 & 0.1472 & 0.5726 & 0.8375 & 0.9348 \\
Photometric Consistency & 0.5348 & 0.3445 & 0.3537 & 0.7358 & 0.1593 & 0.5238 & 0.8095 & 0.9194 \\
Pseudo Labelling & 0.4771 & 0.2821 & 0.2315 & 0.7014 & 0.1488 & 0.5601 & 0.8346 & 0.9349 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.4665 & 0.3125 & 0.2742 & 0.6432 & 0.1483 & 0.5751 & 0.8407 & 0.9332 \\
CrDoCo~\cite{chen2019crdoco} & 0.4466 & 0.2570 & 0.2018 & 0.6819 & 0.1414 & 0.6054 & 0.8504 & 0.9415 \\
Feature Consistency & 0.6060 & 0.3031 & 0.3101 & 0.9231 & 0.2019 & 0.4586 & 0.7172 & 0.8539 \\
Ground-Truth Training & 0.3190 & 0.1985 & 0.1354 & 0.4767 & 0.1094 & 0.7300 & 0.9134 & 0.9682 \\
Ours & 0.4402 & 0.2362 & 0.1878 & 0.6684 & 0.1452 & 0.5806 & 0.8419 & 0.9428
 \\
\bottomrule
\end{tabularx}
}
\caption{Full aggregated results for online adaptation in camera rotations}
\end{table*}


\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.5329 & 0.2800 & 0.3145 & 0.7810 & 0.1890 & 0.5648 & 0.7812 & 0.8697 \\
Schneider et al.~\cite{batchnorm_update} & 0.4277 & 0.2406 & 0.1831 & 0.5946 & 0.1106 & 0.6428 & 0.9373 & 0.9801 \\
Tent~\cite{tent} & 0.5126 & 0.2670 & 0.2860 & 0.8028 & 0.1938 & 0.5829 & 0.7914 & 0.8772 \\
Flip Consistency & 0.4357 & 0.2346 & 0.1864 & 0.6433 & 0.1450 & 0.6331 & 0.8665 & 0.9319 \\
Mask Consistency & 0.5178 & 0.2528 & 0.2424 & 0.7889 & 0.1750 & 0.5784 & 0.7921 & 0.8851 \\
Photometric Consistency & 0.4533 & 0.2537 & 0.2450 & 0.6941 & 0.1634 & 0.6299 & 0.8456 & 0.9163 \\
Pseudo Labelling & 0.3995 & 0.2134 & 0.1594 & 0.6116 & 0.1331 & 0.6853 & 0.8834 & 0.9448 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.3731 & 0.2216 & 0.1649 & 0.5460 & 0.1264 & 0.7014 & 0.9014 & 0.9554 \\
CrDoCo~\cite{chen2019crdoco} & 0.4582 & 0.2349 & 0.1978 & 0.6924 & 0.1495 & 0.6270 & 0.8460 & 0.9207 \\
Feature Consistency & 0.4329 & 0.2269 & 0.1780 & 0.6653 & 0.1418 & 0.6363 & 0.8647 & 0.9400 \\
Ground-Truth Training & 0.2370 & 0.1391 & 0.0800 & 0.3712 & 0.0868 & 0.8339 & 0.9484 & 0.9799 \\
Ours & 0.3143 & 0.1614 & 0.1074 & 0.5047 & 0.1067 & 0.7701 & 0.9262 & 0.9681
 \\
\bottomrule
\end{tabularx}
}
\caption{Full aggregated results for online adaptation in Gaussian noise}
\end{table*}


\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.7756 & 0.4490 & 0.5792 & 1.0052 & 0.1773 & 0.3425 & 0.7521 & 0.9078 \\
Schneider et al.~\cite{batchnorm_update} & 0.4261 & 0.2369 & 0.1779 & 0.5956 & 0.1098 & 0.6539 & 0.9381 & 0.9815 \\
Tent~\cite{tent} & 0.7220 & 0.4178 & 0.5058 & 0.9506 & 0.1706 & 0.3835 & 0.7831 & 0.9205 \\
Flip Consistency & 0.4734 & 0.2967 & 0.2072 & 0.5884 & 0.1308 & 0.4963 & 0.8950 & 0.9699 \\
Mask Consistency & 0.4774 & 0.3051 & 0.2158 & 0.5936 & 0.1344 & 0.4798 & 0.8873 & 0.9661 \\
Photometric Consistency & 0.8657 & 0.5226 & 0.7008 & 1.0652 & 0.1971 & 0.2345 & 0.6882 & 0.8811 \\
Pseudo Labelling & 0.4986 & 0.3126 & 0.2261 & 0.6096 & 0.1349 & 0.4602 & 0.8883 & 0.9669 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.6058 & 0.3934 & 0.3772 & 0.7499 & 0.1620 & 0.4217 & 0.8026 & 0.9305 \\
CrDoCo~\cite{chen2019crdoco} & 0.4115 & 0.2596 & 0.1652 & 0.5325 & 0.1204 & 0.5917 & 0.9140 & 0.9739 \\
Feature Consistency & 0.5007 & 0.2508 & 0.2244 & 0.7620 & 0.1569 & 0.5712 & 0.8241 & 0.9196 \\
Ground-Truth Training & 0.2512 & 0.1471 & 0.0855 & 0.3762 & 0.0830 & 0.8272 & 0.9555 & 0.9855 \\
Ours & 0.3514 & 0.2034 & 0.1313 & 0.4896 & 0.1029 & 0.7025 & 0.9395 & 0.9815
 \\
\bottomrule
\end{tabularx}
}
\caption{Full aggregated results for online adaptation in salt and pepper noise}
\end{table*}


\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.5287 & 0.2896 & 0.3265 & 0.7612 & 0.1785 & 0.5574 & 0.7953 & 0.8889 \\
Schneider et al.~\cite{batchnorm_update} & 0.4343 & 0.2437 & 0.1843 & 0.6044 & 0.1119 & 0.6368 & 0.9342 & 0.9795 \\
Tent~\cite{tent} & 0.5061 & 0.2740 & 0.2866 & 0.7680 & 0.1799 & 0.5765 & 0.8074 & 0.8975 \\
Flip Consistency & 0.4900 & 0.2629 & 0.2202 & 0.6904 & 0.1578 & 0.5531 & 0.8334 & 0.9189 \\
Mask Consistency & 0.4329 & 0.2357 & 0.1770 & 0.6344 & 0.1362 & 0.6195 & 0.8784 & 0.9490 \\
Photometric Consistency & 0.5152 & 0.3087 & 0.3929 & 0.7742 & 0.1784 & 0.5842 & 0.8155 & 0.8960 \\
Pseudo Labelling & 0.4090 & 0.2336 & 0.1734 & 0.6000 & 0.1306 & 0.6469 & 0.8951 & 0.9570 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.3907 & 0.2388 & 0.1782 & 0.5495 & 0.1257 & 0.6660 & 0.9057 & 0.9621 \\
CrDoCo~\cite{chen2019crdoco} & 0.4298 & 0.2324 & 0.1736 & 0.6377 & 0.1346 & 0.6311 & 0.8803 & 0.9496 \\
Feature Consistency & 0.4346 & 0.2324 & 0.1786 & 0.6545 & 0.1395 & 0.6190 & 0.8715 & 0.9466 \\
Ground-Truth Training & 0.2428 & 0.1436 & 0.0822 & 0.3743 & 0.0862 & 0.8303 & 0.9539 & 0.9831 \\
Ours & 0.2990 & 0.1653 & 0.0996 & 0.4604 & 0.0974 & 0.7844 & 0.9456 & 0.9799
 \\
\bottomrule
\end{tabularx}
}
\caption{Full aggregated results for online adaptation in speckle noise}
\end{table*}



==> tables/supp_full_omniscenes.tex <==
\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.4339 & 0.1934 & 0.1418 & 0.6019 & 0.0953 & 0.7367 & 0.9618 & 0.9861 \\
Schneider et al.~\cite{batchnorm_update} & 0.5302 & 0.2057 & 0.2127 & 0.815 & 0.1221 & 0.6679 & 0.9089 & 0.9579 \\
Tent~\cite{tent} & 0.4278 & 0.1906 & 0.1388 & 0.5949 & 0.0943 & 0.7468 & 0.9624 & 0.9863 \\
Flip Consistency & 0.4203 & 0.1863 & 0.1341 & 0.5941 & 0.0917 & 0.7462 & 0.9619 & 0.9864 \\
Mask Consistency & 0.3976 & 0.1745 & 0.1232 & 0.5687 & 0.0883 & 0.7879 & 0.962 & 0.9866 \\
Photometric Consistency & 0.434 & 0.1958 & 0.1404 & 0.6027 & 0.0955 & 0.7235 & 0.9643 & 0.987 \\
Pseudo Labelling & 0.4087 & 0.1819 & 0.1281 & 0.5743 & 0.0909 & 0.7617 & 0.9637 & 0.9873 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.4182 & 0.1781 & 0.1334 & 0.6171 & 0.0921 & 0.7786 & 0.9547 & 0.9839 \\
CrDoCo~\cite{chen2019crdoco} & 0.4099 & 0.1797 & 0.126 & 0.5821 & 0.0907 & 0.7741 & 0.9603 & 0.9864 \\
Feature Consistency & 0.4152 & 0.1768 & 0.1306 & 0.6118 & 0.0915 & 0.7821 & 0.9551 & 0.984 \\
Ground-Truth Training & 0.3161 & 0.1411 & 0.0899 & 0.4893 & 0.0764 & 0.8621 & 0.9758 & 0.991 \\
Ours & 0.3245 & 0.1448 & 0.0928 & 0.4756 & 0.0779 & 0.8686 & 0.9714 & 0.989  \\
\bottomrule
\end{tabularx}
}
\caption{Offline adaptation using 5\% of the panorama images for training in the OmniScenes~\cite{piccolo} dataset.}
\end{table*}

    \smallskip

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.4345 & 0.1951 & 0.1430 & 0.6029 & 0.0953 & 0.7335 & 0.9626 & 0.9866 \\
Schneider et al.~\cite{batchnorm_update} & 0.5317 & 0.2072 & 0.2144 & 0.8169 & 0.1220 & 0.6627 & 0.9087 & 0.9585 \\
Tent~\cite{tent} & 0.4280 & 0.192 & 0.1396 & 0.5957 & 0.0942 & 0.7455 & 0.9634 & 0.9868 \\
Flip Consistency & 0.4044 & 0.1808 & 0.1263 & 0.5743 & 0.0897 & 0.7631 & 0.9633 & 0.9872 \\
Mask Consistency & 0.4022 & 0.1775 & 0.1252 & 0.5732 & 0.0893 & 0.7834 & 0.9612 & 0.9867 \\
Photometric Consistency & 0.4253 & 0.1926 & 0.1367 & 0.5845 & 0.0933 & 0.7364 & 0.9659 & 0.9879 \\
Pseudo Labelling & 0.4167 & 0.1846 & 0.1311 & 0.5907 & 0.0916 & 0.7580 & 0.9630 & 0.9873 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.4210 & 0.1806 & 0.1344 & 0.6210 & 0.0927 & 0.7738 & 0.9536 & 0.9841 \\
CrDoCo~\cite{chen2019crdoco} & 0.4112 & 0.1814 & 0.1274 & 0.5850 & 0.0911 & 0.7719 & 0.9598 & 0.9865 \\
Feature Consistency & 0.4192 & 0.1775 & 0.1335 & 0.6233 & 0.0925 & 0.7794 & 0.9531 & 0.9836 \\
Ground-Truth Training & 0.2981 & 0.1363 & 0.0813 & 0.4543 & 0.0731 & 0.8754 & 0.9793 & 0.9923 \\
Ours & 0.3192 & 0.1434 & 0.0907 & 0.4674 & 0.0767 & 0.8732 & 0.9725 & 0.9896 \\ 
\bottomrule
\end{tabularx}
}
\caption{Offline adaptation using 10\% of the panorama images for training in the OmniScenes~\cite{piccolo} dataset.}
\end{table*}

    \smallskip

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.4334 & 0.1946 & 0.1431 & 0.6030 & 0.0957 & 0.7362 & 0.9616 & 0.9863 \\
Schneider et al.~\cite{batchnorm_update} & 0.4053 & 0.1555 & 0.1368 & 0.7470 & 0.1028 & 0.8033 & 0.9487 & 0.9794 \\
Tent~\cite{tent} & 0.4198 & 0.1848 & 0.1355 & 0.6320 & 0.0955 & 0.7727 & 0.9608 & 0.9859 \\
Flip Consistency & 0.4700 & 0.1903 & 0.1628 & 0.8111 & 0.1059 & 0.7318 & 0.9372 & 0.9742 \\
Mask Consistency & 0.4898 & 0.2069 & 0.1705 & 0.8097 & 0.1095 & 0.6713 & 0.9324 & 0.9731 \\
Photometric Consistency & 0.4498 & 0.2083 & 0.1479 & 0.6656 & 0.1023 & 0.6615 & 0.9555 & 0.9862 \\
Pseudo Labelling & 0.4533 & 0.2043 & 0.1493 & 0.7110 & 0.1035 & 0.6910 & 0.9464 & 0.9801 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.4025 & 0.1767 & 0.1259 & 0.6345 & 0.0936 & 0.7909 & 0.9563 & 0.9831 \\
CrDoCo~\cite{chen2019crdoco} & 0.4989 & 0.2115 & 0.1779 & 0.8306 & 0.1117 & 0.6668 & 0.9311 & 0.9704 \\
Feature Consistency & 0.6594 & 0.2402 & 0.3025 & 1.1390 & 0.1546 & 0.5887 & 0.8267 & 0.9172 \\
Ground-Truth Training & 0.2243 & 0.0922 & 0.0622 & 0.4245 & 0.0619 & 0.9143 & 0.9801 & 0.9930 \\
Ours & 0.3382 & 0.1433 & 0.0989 & 0.5393 & 0.0816 & 0.8432 & 0.9667 & 0.9902
 \\
\bottomrule
\end{tabularx}
}
\caption{Online adaptation in dataset shift evaluated in the OmniScenes~\cite{piccolo} dataset.}
\end{table*}

    \smallskip

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.3766 & 0.2117 & 0.1378 & 0.4868 & 0.0966 & 0.7060 & 0.9715 & 0.9893 \\
Schneider et al.~\cite{batchnorm_update} & 0.3611 & 0.1944 & 0.1115 & 0.4837 & 0.0894 & 0.7520 & 0.9797 & 0.9930 \\
Tent~\cite{tent} & 0.3495 & 0.1977 & 0.1215 & 0.4616 & 0.0938 & 0.7643 & 0.9740 & 0.9901 \\
Flip Consistency & 0.2823 & 0.1727 & 0.0833 & 0.3662 & 0.0850 & 0.8193 & 0.9782 & 0.9925 \\
Mask Consistency & 0.3134 & 0.1999 & 0.0948 & 0.3870 & 0.0940 & 0.7231 & 0.9710 & 0.9918 \\
Photometric Consistency & 0.3486 & 0.2066 & 0.1201 & 0.4373 & 0.0971 & 0.7083 & 0.9714 & 0.9895 \\
Pseudo Labelling & 0.3498 & 0.2166 & 0.1127 & 0.4254 & 0.0983 & 0.6855 & 0.9692 & 0.9910 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.3286 & 0.2126 & 0.1058 & 0.3930 & 0.0975 & 0.7163 & 0.9690 & 0.9911 \\
CrDoCo~\cite{chen2019crdoco} & 0.3268 & 0.2063 & 0.0998 & 0.4068 & 0.0964 & 0.7131 & 0.9682 & 0.9916 \\
Feature Consistency & 0.4863 & 0.2433 & 0.2117 & 0.7122 & 0.1478 & 0.5800 & 0.8350 & 0.9256 \\
Ground-Truth Training & 0.1409 & 0.0835 & 0.0355 & 0.2284 & 0.0548 & 0.9411 & 0.9863 & 0.9948 \\
Ours & 0.1971 & 0.1099 & 0.0498 & 0.3042 & 0.0650 & 0.9132 & 0.9848 & 0.9942 \\
\bottomrule
\end{tabularx}
}
\caption{Online adaptation in low lighting evaluated in the OmniScenes~\cite{piccolo} dataset..}
\end{table*}

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.3929 & 0.2215 & 0.1412 & 0.4980 & 0.1000 & 0.6707 & 0.9686 & 0.9882 \\
Schneider et al.~\cite{batchnorm_update} & 0.3638 & 0.1952 & 0.1113 & 0.4854 & 0.0895 & 0.7459 & 0.9805 & 0.9934 \\
Tent~\cite{tent} & 0.3656 & 0.2072 & 0.1250 & 0.4733 & 0.0974 & 0.7315 & 0.9711 & 0.9891 \\
Flip Consistency & 0.2879 & 0.1727 & 0.0790 & 0.3757 & 0.0858 & 0.8123 & 0.9768 & 0.9919 \\
Mask Consistency & 0.3261 & 0.2037 & 0.0976 & 0.4063 & 0.0958 & 0.7104 & 0.9696 & 0.9913 \\
Photometric Consistency & 0.3948 & 0.2368 & 0.1348 & 0.4736 & 0.1054 & 0.5850 & 0.9678 & 0.9895 \\
Pseudo Labelling & 0.3400 & 0.2120 & 0.1041 & 0.4097 & 0.0973 & 0.7001 & 0.9695 & 0.9911 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.3381 & 0.2128 & 0.1056 & 0.4033 & 0.0968 & 0.7219 & 0.9720 & 0.9915 \\
CrDoCo~\cite{chen2019crdoco} & 0.3301 & 0.2085 & 0.0999 & 0.4066 & 0.0968 & 0.7103 & 0.9690 & 0.9914 \\
Feature Consistency & 0.4502 & 0.2350 & 0.1839 & 0.6507 & 0.1348 & 0.6048 & 0.8644 & 0.9497 \\
Ground-Truth Training & 0.1445 & 0.0850 & 0.0355 & 0.2338 & 0.0560 & 0.9359 & 0.9855 & 0.9944 \\
Ours & 0.2107 & 0.1154 & 0.0519 & 0.3228 & 0.0679 & 0.9006 & 0.9833 & 0.9936
 \\
\bottomrule
\end{tabularx}
}
\caption{Online adaptation in white balance change evaluated in the OmniScenes~\cite{piccolo} dataset..}
\end{table*}

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.3782 & 0.2116 & 0.1269 & 0.4778 & 0.0946 & 0.7262 & 0.9754 & 0.9910 \\
Schneider et al.~\cite{batchnorm_update} & 0.3615 & 0.1941 & 0.1104 & 0.4831 & 0.0891 & 0.7509 & 0.9810 & 0.9934 \\
Tent~\cite{tent} & 0.3474 & 0.1957 & 0.1108 & 0.4477 & 0.0911 & 0.7835 & 0.9776 & 0.9917 \\
Flip Consistency & 0.3026 & 0.1886 & 0.0861 & 0.3696 & 0.0883 & 0.7824 & 0.9791 & 0.9930 \\
Mask Consistency & 0.3281 & 0.2068 & 0.0958 & 0.3980 & 0.0952 & 0.6991 & 0.9736 & 0.9927 \\
Photometric Consistency & 0.3681 & 0.2283 & 0.1267 & 0.4361 & 0.1012 & 0.6431 & 0.9734 & 0.9911 \\
Pseudo Labelling & 0.3248 & 0.2018 & 0.0946 & 0.3890 & 0.0920 & 0.7500 & 0.9768 & 0.9928 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.3031 & 0.1921 & 0.0883 & 0.3667 & 0.0896 & 0.7788 & 0.9782 & 0.9926 \\
CrDoCo~\cite{chen2019crdoco} & 0.3105 & 0.1954 & 0.0886 & 0.3855 & 0.0915 & 0.7581 & 0.9751 & 0.9926 \\
Feature Consistency & 0.3747 & 0.1998 & 0.1324 & 0.5403 & 0.1115 & 0.6917 & 0.9159 & 0.9758 \\
Ground-Truth Training & 0.1354 & 0.0799 & 0.0325 & 0.2215 & 0.0531 & 0.9453 & 0.9875 & 0.9952 \\
Ours & 0.1990 & 0.1080 & 0.0474 & 0.3112 & 0.0648 & 0.9142 & 0.9851 & 0.9942
 \\
\bottomrule
\end{tabularx}
}
\caption{Online adaptation in image gamma change evaluated in the OmniScenes~\cite{piccolo} dataset.}
\end{table*}

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.5290 & 0.1680 & 0.1696 & 0.8141 & 0.0975 & 0.7440 & 0.9399 & 0.9789 \\
Schneider et al.~\cite{batchnorm_update} & 0.7638 & 0.2101 & 0.3221 & 1.3617 & 0.1702 & 0.5857 & 0.8289 & 0.9272 \\
Tent~\cite{tent} & 0.5366 & 0.1678 & 0.1726 & 0.8776 & 0.1014 & 0.7461 & 0.9370 & 0.9780 \\
Flip Consistency & 0.6313 & 0.1721 & 0.2220 & 1.0901 & 0.1132 & 0.7247 & 0.9035 & 0.9601 \\
Mask Consistency & 0.6255 & 0.1745 & 0.2131 & 1.0730 & 0.1093 & 0.7273 & 0.9085 & 0.9662 \\
Photometric Consistency & 0.5512 & 0.1768 & 0.1750 & 0.8885 & 0.1013 & 0.6995 & 0.9405 & 0.9815 \\
Pseudo Labelling & 0.5747 & 0.1737 & 0.1857 & 0.9581 & 0.1025 & 0.7324 & 0.9261 & 0.9764 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.6003 & 0.1687 & 0.2001 & 1.0290 & 0.1061 & 0.7483 & 0.9162 & 0.9690 \\
CrDoCo~\cite{chen2019crdoco} & 0.6517 & 0.1825 & 0.2295 & 1.1306 & 0.1132 & 0.7116 & 0.9027 & 0.9617 \\
Feature Consistency & 0.8238 & 0.2163 & 0.3541 & 1.4397 & 0.1496 & 0.6082 & 0.8331 & 0.9258 \\
Ground-Truth Training & 0.3663 & 0.1147 & 0.1058 & 0.6516 & 0.0739 & 0.8773 & 0.9708 & 0.9898 \\
Ours & 0.4790 & 0.1494 & 0.1435 & 0.7819 & 0.0911 & 0.8029 & 0.9510 & 0.9855
 \\
\bottomrule
\end{tabularx}
}
\caption{Online adaptation in large scenes evaluated in the OmniScenes~\cite{piccolo} dataset.}
\end{table*}

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.2921 & 0.1454 & 0.0738 & 0.4064 & 0.0750 & 0.8674 & 0.9787 & 0.9931 \\
Schneider et al.~\cite{batchnorm_update} & 0.2907 & 0.1388 & 0.0691 & 0.4183 & 0.0718 & 0.8625 & 0.9874 & 0.9954 \\
Tent~\cite{tent} & 0.2862 & 0.1424 & 0.0710 & 0.4029 & 0.0752 & 0.8730 & 0.9794 & 0.9934 \\
Flip Consistency & 0.2898 & 0.1499 & 0.0699 & 0.3888 & 0.0758 & 0.8549 & 0.9832 & 0.9946 \\
Mask Consistency & 0.2459 & 0.1317 & 0.0540 & 0.3321 & 0.0693 & 0.8851 & 0.9863 & 0.9954 \\
Photometric Consistency & 0.2560 & 0.1302 & 0.0587 & 0.3583 & 0.0702 & 0.8889 & 0.9831 & 0.9943 \\
Pseudo Labelling & 0.2732 & 0.1407 & 0.0624 & 0.3699 & 0.0716 & 0.8783 & 0.9857 & 0.9953 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.2453 & 0.1328 & 0.0542 & 0.3300 & 0.0698 & 0.8819 & 0.9860 & 0.9953 \\
CrDoCo~\cite{chen2019crdoco} & 0.2353 & 0.1269 & 0.0503 & 0.3216 & 0.0676 & 0.8905 & 0.9863 & 0.9953 \\
Feature Consistency & 0.2665 & 0.1283 & 0.0606 & 0.3835 & 0.0763 & 0.8547 & 0.9759 & 0.9904 \\
Ground-Truth Training & 0.1809 & 0.0930 & 0.0343 & 0.2679 & 0.0562 & 0.9325 & 0.9877 & 0.9954 \\
Ours & 0.2121 & 0.1058 & 0.0428 & 0.3119 & 0.0624 & 0.9139 & 0.9857 & 0.9946
 \\
\bottomrule
\end{tabularx}
}
\caption{Online adaptation in small scenes evaluated in the OmniScenes~\cite{piccolo} dataset.}
\end{table*}


\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.4585 & 0.2720 & 0.2294 & 0.6489 & 0.1443 & 0.5798 & 0.8498 & 0.9426 \\
Schneider et al.~\cite{batchnorm_update} & 0.4867 & 0.2878 & 0.2346 & 0.6636 & 0.1491 & 0.5088 & 0.8310 & 0.9432 \\
Tent~\cite{tent} & 0.4419 & 0.2570 & 0.2021 & 0.6299 & 0.1413 & 0.5924 & 0.8583 & 0.9469 \\
Flip Consistency & 0.4128 & 0.2389 & 0.1609 & 0.6048 & 0.1270 & 0.6184 & 0.8907 & 0.9652 \\
Mask Consistency & 0.4368 & 0.2358 & 0.1746 & 0.6737 & 0.1352 & 0.6165 & 0.8678 & 0.9526 \\
Photometric Consistency & 0.4316 & 0.2574 & 0.1929 & 0.6076 & 0.1338 & 0.5979 & 0.8788 & 0.9593 \\
Pseudo Labelling & 0.4421 & 0.2413 & 0.1786 & 0.6687 & 0.1364 & 0.6013 & 0.8667 & 0.9536 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.4044 & 0.2565 & 0.1891 & 0.5642 & 0.1298 & 0.6314 & 0.8880 & 0.9613 \\
CrDoCo~\cite{chen2019crdoco} & 0.4214 & 0.2265 & 0.1668 & 0.6600 & 0.1314 & 0.6457 & 0.8741 & 0.9555 \\
Feature Consistency & 0.6067 & 0.2913 & 0.2990 & 0.9284 & 0.2001 & 0.4699 & 0.7231 & 0.8552 \\
Ground-Truth Training & 0.2604 & 0.1583 & 0.0864 & 0.3917 & 0.0916 & 0.7987 & 0.9488 & 0.9833 \\
Ours & 0.4089 & 0.2106 & 0.1486 & 0.6182 & 0.1324 & 0.6070 & 0.8686 & 0.9593
 \\
\bottomrule
\end{tabularx}
}
\caption{Online adaptation in camera rotations evaluated in the OmniScenes~\cite{piccolo} dataset.}
\end{table*}


\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.5029 & 0.2770 & 0.3114 & 0.7194 & 0.1768 & 0.5950 & 0.8021 & 0.8799 \\
Schneider et al.~\cite{batchnorm_update} & 0.3800 & 0.2071 & 0.1240 & 0.5075 & 0.0953 & 0.7070 & 0.9723 & 0.9914 \\
Tent~\cite{tent} & 0.4718 & 0.2585 & 0.2693 & 0.7245 & 0.1812 & 0.6205 & 0.8183 & 0.8916 \\
Flip Consistency & 0.3416 & 0.2064 & 0.1161 & 0.4584 & 0.1090 & 0.7121 & 0.9401 & 0.9753 \\
Mask Consistency & 0.3818 & 0.2004 & 0.1404 & 0.5899 & 0.1245 & 0.7092 & 0.9015 & 0.9578 \\
Photometric Consistency & 0.4544 & 0.2597 & 0.2660 & 0.6843 & 0.1672 & 0.6366 & 0.8445 & 0.9097 \\
Pseudo Labelling & 0.3274 & 0.1854 & 0.1078 & 0.4754 & 0.1070 & 0.7623 & 0.9339 & 0.9721 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.3324 & 0.2043 & 0.1369 & 0.4648 & 0.1126 & 0.7495 & 0.9298 & 0.9681 \\
CrDoCo~\cite{chen2019crdoco} & 0.3383 & 0.1929 & 0.1102 & 0.4906 & 0.1051 & 0.7404 & 0.9408 & 0.9781 \\
Feature Consistency & 0.4046 & 0.2115 & 0.1539 & 0.6142 & 0.1302 & 0.6660 & 0.8876 & 0.9531 \\
Ground-Truth Training & 0.1868 & 0.1096 & 0.0550 & 0.2947 & 0.0720 & 0.8907 & 0.9674 & 0.9860 \\
Ours & 0.2557 & 0.1349 & 0.0717 & 0.4037 & 0.0851 & 0.8445 & 0.9597 & 0.9837
 \\
\bottomrule
\end{tabularx}
}
\caption{Online adaptation in gaussian noise evaluated in the OmniScenes~\cite{piccolo} dataset.}
\end{table*}


\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.7473 & 0.4189 & 0.4784 & 0.9412 & 0.1649 & 0.3244 & 0.7849 & 0.9368 \\
Schneider et al.~\cite{batchnorm_update} & 0.3805 & 0.2064 & 0.1217 & 0.5048 & 0.0948 & 0.7144 & 0.9723 & 0.9923 \\
Tent~\cite{tent} & 0.6900 & 0.3872 & 0.4067 & 0.8798 & 0.1576 & 0.3752 & 0.8195 & 0.9481 \\
Flip Consistency & 0.4892 & 0.3025 & 0.2027 & 0.5750 & 0.1281 & 0.4454 & 0.9114 & 0.9793 \\
Mask Consistency & 0.4715 & 0.2995 & 0.1914 & 0.5531 & 0.1281 & 0.4464 & 0.9129 & 0.9799 \\
Photometric Consistency & 0.7913 & 0.4655 & 0.4944 & 0.9309 & 0.1776 & 0.1959 & 0.7345 & 0.9340 \\
Pseudo Labelling & 0.4980 & 0.3064 & 0.2038 & 0.5793 & 0.1286 & 0.4273 & 0.9164 & 0.9803 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.5771 & 0.3668 & 0.3141 & 0.6923 & 0.1511 & 0.4214 & 0.8409 & 0.9531 \\
CrDoCo~\cite{chen2019crdoco} & 0.4024 & 0.2534 & 0.1463 & 0.4898 & 0.1130 & 0.5797 & 0.9392 & 0.9852 \\
Feature Consistency & 0.4755 & 0.2377 & 0.1979 & 0.7094 & 0.1417 & 0.5922 & 0.8486 & 0.9376 \\
Ground-Truth Training & 0.2030 & 0.1171 & 0.0575 & 0.3034 & 0.0677 & 0.8789 & 0.9764 & 0.9925 \\
Ours & 0.3311 & 0.1876 & 0.1080 & 0.4455 & 0.0930 & 0.7160 & 0.9620 & 0.9905
 \\
\bottomrule
\end{tabularx}
}
\caption{Online adaptation in salt and pepper noise evaluated in the OmniScenes~\cite{piccolo} dataset.}
\end{table*}


\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.5285 & 0.2970 & 0.3467 & 0.7498 & 0.1787 & 0.5729 & 0.8000 & 0.8826 \\
Schneider et al.~\cite{batchnorm_update} & 0.3918 & 0.2119 & 0.1344 & 0.5313 & 0.0981 & 0.7048 & 0.9646 & 0.9890 \\
Tent~\cite{tent} & 0.4945 & 0.2753 & 0.2902 & 0.7334 & 0.1783 & 0.5988 & 0.8170 & 0.8958 \\
Flip Consistency & 0.3779 & 0.2323 & 0.1408 & 0.4878 & 0.1154 & 0.6493 & 0.9347 & 0.9751 \\
Mask Consistency & 0.3641 & 0.2137 & 0.1273 & 0.5021 & 0.1117 & 0.6906 & 0.9327 & 0.9764 \\
Photometric Consistency & 0.5642 & 0.3368 & 0.4919 & 0.8553 & 0.2010 & 0.5685 & 0.7775 & 0.8630 \\
Pseudo Labelling & 0.3761 & 0.2233 & 0.1510 & 0.5260 & 0.1182 & 0.6849 & 0.9232 & 0.9695 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.3691 & 0.2299 & 0.1603 & 0.4953 & 0.1169 & 0.6954 & 0.9246 & 0.9698 \\
CrDoCo~\cite{chen2019crdoco} & 0.3581 & 0.2093 & 0.1233 & 0.5006 & 0.1096 & 0.7097 & 0.9355 & 0.9771 \\
Feature Consistency & 0.4086 & 0.2218 & 0.1542 & 0.5971 & 0.1280 & 0.6413 & 0.8958 & 0.9611 \\
Ground-Truth Training & 0.2036 & 0.1194 & 0.0602 & 0.3150 & 0.0744 & 0.8745 & 0.9683 & 0.9878 \\
Ours & 0.2753 & 0.1509 & 0.0830 & 0.4160 & 0.0881 & 0.8233 & 0.9603 & 0.9850
 \\
\bottomrule
\end{tabularx}
}
\caption{Online adaptation in speckle noise evaluated in the OmniScenes~\cite{piccolo} dataset.}
\end{table*}



==> tables/supp_full_stanford.tex <==
\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.4656 & 0.2533 & 0.2171 & 0.6551 & 0.1215 & 0.63 & 0.9077 & 0.9704 \\
Schneider et al.~\cite{batchnorm_update} & 0.5102 & 0.2684 & 0.2686 & 0.7714 & 0.1308 & 0.5776 & 0.8871 & 0.9632 \\
Tent~\cite{tent} & 0.4645 & 0.2527 & 0.2163 & 0.6537 & 0.1213 & 0.6314 & 0.908 & 0.9705 \\
Flip Consistency & 0.4586 & 0.2494 & 0.2085 & 0.6441 & 0.1207 & 0.6344 & 0.9091 & 0.9706 \\
Mask Consistency & 0.444 & 0.2426 & 0.1967 & 0.6271 & 0.118 & 0.6522 & 0.914 & 0.9722 \\
Photometric Consistency & 0.4674 & 0.2559 & 0.2188 & 0.6538 & 0.1218 & 0.6254 & 0.9071 & 0.9706 \\
Pseudo Labelling & 0.4476 & 0.2471 & 0.2006 & 0.6214 & 0.1179 & 0.6411 & 0.9133 & 0.9732 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.4404 & 0.2402 & 0.1944 & 0.6268 & 0.1183 & 0.6565 & 0.9136 & 0.9716 \\
CrDoCo~\cite{chen2019crdoco} & 0.444 & 0.2437 & 0.1971 & 0.6257 & 0.1181 & 0.6497 & 0.9134 & 0.9722 \\
Feature Consistency & 0.4374 & 0.2365 & 0.19 & 0.6223 & 0.1172 & 0.6611 & 0.9155 & 0.9722 \\
Ground-Truth Training & 0.4023 & 0.2234 & 0.1678 & 0.5646 & 0.1108 & 0.6903 & 0.9252 & 0.9762 \\
Ours & 0.4313 & 0.2365 & 0.1896 & 0.6057 & 0.1152 & 0.6652 & 0.9185 & 0.9744 \\
\bottomrule
\end{tabularx}
}
\caption{Offline adaptation using 5\% of the panorama images for training in the Stanford 2D-3D-S~\cite{stanford2d3d} dataset.}
\end{table*}

    \smallskip

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.4601 & 0.2491 & 0.2136 & 0.6560 & 0.1217 & 0.6387 & 0.9091 & 0.9698 \\
Schneider et al.~\cite{batchnorm_update} & 0.4973 & 0.2618 & 0.2557 & 0.7548 & 0.1276 & 0.5865 & 0.8957 & 0.9662 \\
Tent~\cite{tent} & 0.4592 & 0.2486 & 0.2129 & 0.6549 & 0.1215 & 0.6398 & 0.9094 & 0.9699 \\
Flip Consistency & 0.4513 & 0.2461 & 0.2051 & 0.6383 & 0.1202 & 0.6435 & 0.9115 & 0.9706 \\
Mask Consistency & 0.4461 & 0.2411 & 0.2004 & 0.6419 & 0.1197 & 0.6554 & 0.9124 & 0.9702 \\
Photometric Consistency & 0.4623 & 0.2510 & 0.2152 & 0.6573 & 0.1220 & 0.6352 & 0.9085 & 0.9698 \\
Pseudo Labelling & 0.4505 & 0.2448 & 0.2038 & 0.6431 & 0.1206 & 0.6452 & 0.9108 & 0.9701 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.4430 & 0.2385 & 0.1983 & 0.6419 & 0.1198 & 0.6610 & 0.9120 & 0.9694 \\
CrDoCo~\cite{chen2019crdoco} & 0.4444 & 0.2419 & 0.1991 & 0.6362 & 0.1191 & 0.6537 & 0.9131 & 0.9711 \\
Feature Consistency & 0.4415 & 0.2378 & 0.1971 & 0.6385 & 0.1196 & 0.6618 & 0.9116 & 0.9693 \\
Ground-Truth Training & 0.4073 & 0.2255 & 0.1741 & 0.5789 & 0.1126 & 0.6881 & 0.9236 & 0.9749 \\
Ours & 0.4313 & 0.2350 & 0.1914 & 0.6134 & 0.1168 & 0.6686 & 0.9164 & 0.9722 \\
\bottomrule
\end{tabularx}
}
\caption{Offline adaptation using 10\% of the panorama images for training in the Stanford 2D-3D-S~\cite{stanford2d3d} dataset.}
\end{table*}

    \smallskip

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.4538 & 0.2461 & 0.2069 & 0.6504 & 0.1208 & 0.6444 & 0.9113 & 0.9708 \\
Schneider et al.~\cite{batchnorm_update} & 0.4381 & 0.2351 & 0.1957 & 0.6793 & 0.1156 & 0.6446 & 0.9266 & 0.9780 \\
Tent~\cite{tent} & 0.4397 & 0.2361 & 0.1949 & 0.6680 & 0.1209 & 0.6683 & 0.9159 & 0.9718 \\
Flip Consistency & 0.3951 & 0.2253 & 0.1538 & 0.6183 & 0.1145 & 0.6785 & 0.9221 & 0.9750 \\
Mask Consistency & 0.4120 & 0.2333 & 0.1638 & 0.6594 & 0.1186 & 0.6552 & 0.9152 & 0.9709 \\
Photometric Consistency & 0.4752 & 0.2792 & 0.2150 & 0.6596 & 0.1277 & 0.5670 & 0.9030 & 0.9718 \\
Pseudo Labelling & 0.4038 & 0.2304 & 0.1608 & 0.6329 & 0.1165 & 0.6684 & 0.9186 & 0.9729 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.4017 & 0.2336 & 0.1683 & 0.6236 & 0.1166 & 0.6762 & 0.9156 & 0.9726 \\
CrDoCo~\cite{chen2019crdoco} & 0.4091 & 0.2313 & 0.1644 & 0.6626 & 0.1175 & 0.6654 & 0.9137 & 0.9714 \\
Feature Consistency & 0.6116 & 0.2687 & 0.3168 & 1.0522 & 0.1906 & 0.5360 & 0.7803 & 0.8794 \\
Ground-Truth Training & 0.2624 & 0.1415 & 0.0921 & 0.4524 & 0.0866 & 0.8366 & 0.9585 & 0.9860 \\
Ours & 0.2994 & 0.1594 & 0.1136 & 0.5008 & 0.0944 & 0.8086 & 0.9511 & 0.9824
 \\
\bottomrule
\end{tabularx}
}
\caption{Online adaptation in dataset shift evaluated in the Stanford 2D-3D-S~\cite{stanford2d3d} dataset.}
\end{table*}

    \smallskip

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.4018 & 0.2295 & 0.1645 & 0.5567 & 0.1157 & 0.6505 & 0.9194 & 0.9743 \\
Schneider et al.~\cite{batchnorm_update} & 0.4826 & 0.2759 & 0.2379 & 0.6949 & 0.1263 & 0.5577 & 0.9031 & 0.9725 \\
Tent~\cite{tent} & 0.3910 & 0.2225 & 0.1565 & 0.5652 & 0.1157 & 0.6682 & 0.9220 & 0.9749 \\
Flip Consistency & 0.3391 & 0.2086 & 0.1213 & 0.4775 & 0.1091 & 0.7039 & 0.9281 & 0.9774 \\
Mask Consistency & 0.3427 & 0.2140 & 0.1234 & 0.4817 & 0.1100 & 0.6942 & 0.9258 & 0.9769 \\
Photometric Consistency & 0.3874 & 0.2238 & 0.1527 & 0.5597 & 0.1188 & 0.6626 & 0.9179 & 0.9720 \\
Pseudo Labelling & 0.3671 & 0.2306 & 0.1411 & 0.5012 & 0.1136 & 0.6662 & 0.9213 & 0.9765 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.3670 & 0.2360 & 0.1464 & 0.4988 & 0.1158 & 0.6636 & 0.9150 & 0.9735 \\
CrDoCo~\cite{chen2019crdoco} & 0.3475 & 0.2109 & 0.1240 & 0.5055 & 0.1116 & 0.6933 & 0.9216 & 0.9751 \\
Feature Consistency & 0.4633 & 0.2501 & 0.2024 & 0.7093 & 0.1484 & 0.5870 & 0.8515 & 0.9350 \\
Ground-Truth Training & 0.2728 & 0.1594 & 0.0853 & 0.4119 & 0.0932 & 0.7954 & 0.9498 & 0.9851 \\
Ours & 0.2995 & 0.1712 & 0.1001 & 0.4517 & 0.0987 & 0.7696 & 0.9440 & 0.9815 \\
\bottomrule
\end{tabularx}
}
\caption{Online adaptation in low lighting evaluated in the Stanford 2D-3D-S~\cite{stanford2d3d} dataset..}
\end{table*}

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.4484 & 0.2503 & 0.1943 & 0.6187 & 0.1289 & 0.6043 & 0.8947 & 0.9617 \\
Schneider et al.~\cite{batchnorm_update} & 0.4819 & 0.2749 & 0.2358 & 0.6904 & 0.1259 & 0.5581 & 0.9036 & 0.9731 \\
Tent~\cite{tent} & 0.4364 & 0.2426 & 0.1856 & 0.6328 & 0.1305 & 0.6231 & 0.8982 & 0.9622 \\
Flip Consistency & 0.3763 & 0.2190 & 0.1448 & 0.5630 & 0.1237 & 0.6775 & 0.9015 & 0.9626 \\
Mask Consistency & 0.3567 & 0.2250 & 0.1324 & 0.4933 & 0.1130 & 0.6819 & 0.9193 & 0.9755 \\
Photometric Consistency & 0.4583 & 0.2692 & 0.2000 & 0.6268 & 0.1314 & 0.5745 & 0.8938 & 0.9657 \\
Pseudo Labelling & 0.4116 & 0.2579 & 0.1670 & 0.5454 & 0.1225 & 0.6046 & 0.9069 & 0.9725 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.3934 & 0.2481 & 0.1597 & 0.5294 & 0.1200 & 0.6352 & 0.9087 & 0.9729 \\
CrDoCo~\cite{chen2019crdoco} & 0.3506 & 0.2190 & 0.1276 & 0.4926 & 0.1119 & 0.6902 & 0.9202 & 0.9761 \\
Feature Consistency & 0.5548 & 0.2730 & 0.2651 & 0.8570 & 0.1847 & 0.5144 & 0.7729 & 0.8830 \\
Ground-Truth Training & 0.2680 & 0.1574 & 0.0842 & 0.4079 & 0.0921 & 0.8039 & 0.9501 & 0.9849 \\
Ours & 0.3208 & 0.1779 & 0.1121 & 0.4968 & 0.1084 & 0.7516 & 0.9292 & 0.9736
 \\
\bottomrule
\end{tabularx}
}
\caption{Online adaptation in white balance change evaluated in the Stanford 2D-3D-S~\cite{stanford2d3d} dataset.}
\end{table*}

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.4480 & 0.2630 & 0.2045 & 0.6001 & 0.1214 & 0.6096 & 0.9060 & 0.9729 \\
Schneider et al.~\cite{batchnorm_update} & 0.4787 & 0.2730 & 0.2278 & 0.6811 & 0.1247 & 0.5567 & 0.9056 & 0.9743 \\
Tent~\cite{tent} & 0.4306 & 0.2524 & 0.1906 & 0.5968 & 0.1201 & 0.6343 & 0.9117 & 0.9745 \\
Flip Consistency & 0.3722 & 0.2373 & 0.1459 & 0.4994 & 0.1144 & 0.6608 & 0.9186 & 0.9767 \\
Mask Consistency & 0.3439 & 0.2207 & 0.1275 & 0.4743 & 0.1098 & 0.6949 & 0.9245 & 0.9777 \\
Photometric Consistency & 0.5021 & 0.3105 & 0.2447 & 0.6446 & 0.1357 & 0.5093 & 0.8789 & 0.9662 \\
Pseudo Labelling & 0.3923 & 0.2499 & 0.1577 & 0.5182 & 0.1178 & 0.6302 & 0.9145 & 0.9757 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.3835 & 0.2490 & 0.1601 & 0.5140 & 0.1187 & 0.6445 & 0.9090 & 0.9732 \\
CrDoCo~\cite{chen2019crdoco} & 0.3575 & 0.2325 & 0.1391 & 0.4880 & 0.1137 & 0.6727 & 0.9164 & 0.9759 \\
Feature Consistency & 0.4370 & 0.2273 & 0.1832 & 0.6742 & 0.1415 & 0.6208 & 0.8598 & 0.9396 \\
Ground-Truth Training & 0.2600 & 0.1526 & 0.0836 & 0.4019 & 0.0900 & 0.8167 & 0.9527 & 0.9854 \\
Ours & 0.2887 & 0.1678 & 0.0993 & 0.4387 & 0.0956 & 0.7895 & 0.9468 & 0.9826
 \\
\bottomrule
\end{tabularx}
}
\caption{Online adaptation in image gamma change evaluated in the Stanford 2D-3D-S~\cite{stanford2d3d} dataset.}
\end{table*}

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.4477 & 0.2187 & 0.2015 & 0.6987 & 0.1164 & 0.7078 & 0.9259 & 0.9698 \\
Schneider et al.~\cite{batchnorm_update} & 0.3996 & 0.1865 & 0.1607 & 0.6796 & 0.1048 & 0.7645 & 0.9473 & 0.9806 \\
Tent~\cite{tent} & 0.4541 & 0.2178 & 0.2011 & 0.7520 & 0.1204 & 0.7067 & 0.9253 & 0.9696 \\
Flip Consistency & 0.4345 & 0.2180 & 0.1738 & 0.7062 & 0.1110 & 0.7038 & 0.9382 & 0.9784 \\
Mask Consistency & 0.4330 & 0.2170 & 0.1749 & 0.7296 & 0.1110 & 0.7044 & 0.9361 & 0.9776 \\
Photometric Consistency & 0.4519 & 0.2170 & 0.1975 & 0.7504 & 0.1214 & 0.6990 & 0.9260 & 0.9686 \\
Pseudo Labelling & 0.4341 & 0.2070 & 0.1745 & 0.7638 & 0.1136 & 0.7193 & 0.9303 & 0.9734 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.4243 & 0.2060 & 0.1698 & 0.7484 & 0.1096 & 0.7282 & 0.9350 & 0.9763 \\
CrDoCo~\cite{chen2019crdoco} & 0.4212 & 0.2017 & 0.1665 & 0.7592 & 0.1082 & 0.7390 & 0.9356 & 0.9767 \\
Feature Consistency & 0.5788 & 0.2286 & 0.2871 & 1.1030 & 0.1693 & 0.6357 & 0.8420 & 0.9113 \\
Ground-Truth Training & 0.3121 & 0.1561 & 0.1243 & 0.5452 & 0.0894 & 0.8356 & 0.9605 & 0.9852 \\
Ours & 0.3471 & 0.1727 & 0.1423 & 0.5803 & 0.0960 & 0.8036 & 0.9546 & 0.9829
 \\
\bottomrule
\end{tabularx}
}
\caption{Online adaptation in large scenes evaluated in the Stanford 2D-3D-S~\cite{stanford2d3d} dataset.}
\end{table*}

\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.3692 & 0.2702 & 0.1673 & 0.4963 & 0.1289 & 0.5536 & 0.8942 & 0.9700 \\
Schneider et al.~\cite{batchnorm_update} & 0.7259 & 0.5169 & 0.5504 & 0.9410 & 0.1914 & 0.1590 & 0.6832 & 0.9222 \\
Tent~\cite{tent} & 0.3686 & 0.2684 & 0.1670 & 0.5025 & 0.1292 & 0.5605 & 0.8937 & 0.9693 \\
Flip Consistency & 0.3494 & 0.2575 & 0.1489 & 0.4742 & 0.1277 & 0.5780 & 0.8986 & 0.9681 \\
Mask Consistency & 0.3504 & 0.2614 & 0.1492 & 0.4681 & 0.1254 & 0.5726 & 0.9052 & 0.9717 \\
Photometric Consistency & 0.3900 & 0.2870 & 0.1836 & 0.5210 & 0.1318 & 0.5234 & 0.8856 & 0.9683 \\
Pseudo Labelling & 0.3788 & 0.2817 & 0.1737 & 0.5015 & 0.1298 & 0.5329 & 0.8933 & 0.9700 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.3598 & 0.2692 & 0.1584 & 0.4775 & 0.1271 & 0.5572 & 0.9006 & 0.9705 \\
CrDoCo~\cite{chen2019crdoco} & 0.3441 & 0.2565 & 0.1442 & 0.4637 & 0.1269 & 0.5813 & 0.8997 & 0.9684 \\
Feature Consistency & 0.3518 & 0.2558 & 0.1492 & 0.4838 & 0.1312 & 0.5715 & 0.8899 & 0.9635 \\
Ground-Truth Training & 0.3224 & 0.2387 & 0.1324 & 0.4428 & 0.1204 & 0.6365 & 0.9131 & 0.9731 \\
Ours & 0.3380 & 0.2485 & 0.1400 & 0.4612 & 0.1240 & 0.6030 & 0.9069 & 0.9717
 \\
\bottomrule
\end{tabularx}
}
\caption{Online adaptation in small scenes evaluated in the Stanford 2D-3D-S~\cite{stanford2d3d} dataset.}
\end{table*}


\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.6338 & 0.4173 & 0.5105 & 0.8961 & 0.1883 & 0.4565 & 0.7385 & 0.8736 \\
Schneider et al.~\cite{batchnorm_update} & 0.6689 & 0.4128 & 0.5905 & 1.0118 & 0.1957 & 0.4283 & 0.7307 & 0.8763 \\
Tent~\cite{tent} & 0.6140 & 0.4044 & 0.4817 & 0.8734 & 0.1863 & 0.4710 & 0.7482 & 0.8805 \\
Flip Consistency & 0.5165 & 0.3283 & 0.2912 & 0.7463 & 0.1654 & 0.5099 & 0.7931 & 0.9093 \\
Mask Consistency & 0.5241 & 0.3456 & 0.3090 & 0.7420 & 0.1666 & 0.5014 & 0.7883 & 0.9060 \\
Photometric Consistency & 0.7020 & 0.4857 & 0.6141 & 0.9436 & 0.2006 & 0.4037 & 0.6973 & 0.8547 \\
Pseudo Labelling & 0.5337 & 0.3482 & 0.3172 & 0.7543 & 0.1689 & 0.4933 & 0.7826 & 0.9045 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.5671 & 0.4031 & 0.4120 & 0.7711 & 0.1782 & 0.4838 & 0.7641 & 0.8876 \\
CrDoCo~\cite{chen2019crdoco} & 0.4875 & 0.3064 & 0.2586 & 0.7175 & 0.1576 & 0.5402 & 0.8119 & 0.9189 \\
Feature Consistency & 0.6049 & 0.3223 & 0.3282 & 0.9144 & 0.2048 & 0.4404 & 0.7076 & 0.8517 \\
Ground-Truth Training & 0.4140 & 0.2637 & 0.2149 & 0.6145 & 0.1382 & 0.6188 & 0.8560 & 0.9437 \\
Ours & 0.4910 & 0.2778 & 0.2513 & 0.7496 & 0.1659 & 0.5379 & 0.7986 & 0.9162
 \\
\bottomrule
\end{tabularx}
}
\caption{Online adaptation in camera rotations evaluated in the Stanford 2D-3D-S~\cite{stanford2d3d} dataset.}
\end{table*}


\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.5816 & 0.2848 & 0.3196 & 0.8809 & 0.2088 & 0.5158 & 0.7474 & 0.8531 \\
Schneider et al.~\cite{batchnorm_update} & 0.5049 & 0.2948 & 0.2788 & 0.7356 & 0.1354 & 0.5389 & 0.8807 & 0.9617 \\
Tent~\cite{tent} & 0.5788 & 0.2808 & 0.3131 & 0.9297 & 0.2143 & 0.5220 & 0.7478 & 0.8540 \\
Flip Consistency & 0.5882 & 0.2802 & 0.3002 & 0.9428 & 0.2032 & 0.5052 & 0.7474 & 0.8617 \\
Mask Consistency & 0.7381 & 0.3376 & 0.4076 & 1.1113 & 0.2568 & 0.3664 & 0.6149 & 0.7674 \\
Photometric Consistency & 0.4515 & 0.2441 & 0.2110 & 0.7100 & 0.1573 & 0.6191 & 0.8474 & 0.9269 \\
Pseudo Labelling & 0.5162 & 0.2587 & 0.2430 & 0.8323 & 0.1755 & 0.5605 & 0.8016 & 0.9005 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.4390 & 0.2497 & 0.2102 & 0.6776 & 0.1487 & 0.6234 & 0.8554 & 0.9349 \\
CrDoCo~\cite{chen2019crdoco} & 0.6525 & 0.3030 & 0.3396 & 1.0192 & 0.2214 & 0.4432 & 0.6924 & 0.8277 \\
Feature Consistency & 0.4787 & 0.2518 & 0.2171 & 0.7482 & 0.1605 & 0.5882 & 0.8276 & 0.9187 \\
Ground-Truth Training & 0.3183 & 0.1869 & 0.1206 & 0.4952 & 0.1109 & 0.7418 & 0.9176 & 0.9701 \\
Ours & 0.4091 & 0.2044 & 0.1651 & 0.6682 & 0.1417 & 0.6495 & 0.8719 & 0.9427
 \\
\bottomrule
\end{tabularx}
}
\caption{Online adaptation in gaussian noise evaluated in the Stanford 2D-3D-S~\cite{stanford2d3d} dataset.}
\end{table*}


\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.8215 & 0.4977 & 0.7425 & 1.1088 & 0.1973 & 0.3717 & 0.6989 & 0.8608 \\
Schneider et al.~\cite{batchnorm_update} & 0.5000 & 0.2864 & 0.2689 & 0.7428 & 0.1341 & 0.5560 & 0.8826 & 0.9641 \\
Tent~\cite{tent} & 0.7739 & 0.4674 & 0.6664 & 1.0653 & 0.1916 & 0.3970 & 0.7241 & 0.8759 \\
Flip Consistency & 0.4477 & 0.2872 & 0.2146 & 0.6100 & 0.1353 & 0.5787 & 0.8684 & 0.9546 \\
Mask Consistency & 0.4869 & 0.3141 & 0.2554 & 0.6591 & 0.1445 & 0.5340 & 0.8458 & 0.9437 \\
Photometric Consistency & 0.9862 & 0.6152 & 1.0352 & 1.2827 & 0.2288 & 0.2971 & 0.6131 & 0.7955 \\
Pseudo Labelling & 0.4995 & 0.3226 & 0.2622 & 0.6586 & 0.1451 & 0.5136 & 0.8429 & 0.9453 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.6522 & 0.4365 & 0.4794 & 0.8433 & 0.1797 & 0.4222 & 0.7406 & 0.8938 \\
CrDoCo~\cite{chen2019crdoco} & 0.4263 & 0.2697 & 0.1957 & 0.6018 & 0.1323 & 0.6111 & 0.8732 & 0.9557 \\
Feature Consistency & 0.5416 & 0.2721 & 0.2674 & 0.8473 & 0.1814 & 0.5372 & 0.7844 & 0.8905 \\
Ground-Truth Training & 0.3294 & 0.1957 & 0.1308 & 0.4940 & 0.1077 & 0.7434 & 0.9217 & 0.9741 \\
Ours & 0.3843 & 0.2290 & 0.1690 & 0.5610 & 0.1189 & 0.6806 & 0.9031 & 0.9670
 \\
\bottomrule
\end{tabularx}
}
\caption{Online adaptation in salt and pepper noise evaluated in the Stanford 2D-3D-S~\cite{stanford2d3d} dataset.}
\end{table*}


\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabularx}{2.5\columnwidth}{l|YYYYYYYY}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{MAE} & \multirow{2}{*}{Abs. Rel.} & \multirow{2}{*}{Sq. Rel.} & \multirow{2}{*}{RMSE} & \multirow{2}{*}{RMSE (Log)} & Inlier Ratio & Inlier Ratio & Inlier Ratio \\
& & & & & & ($\lambda=1.25$) & ($\lambda=1.25^2$)& ($\lambda=1.25^3$)\\
\midrule
No Adaptation & 0.5291 & 0.2777 & 0.2937 & 0.7796 & 0.1783 & 0.5324 & 0.7877 & 0.8992 \\
Schneider et al.~\cite{batchnorm_update} & 0.5032 & 0.2953 & 0.2651 & 0.7229 & 0.1342 & 0.5266 & 0.8850 & 0.9642 \\
Tent~\cite{tent} & 0.5250 & 0.2719 & 0.2807 & 0.8240 & 0.1824 & 0.5404 & 0.7918 & 0.9003 \\
Flip Consistency & 0.6716 & 0.3124 & 0.3487 & 1.0187 & 0.2264 & 0.3972 & 0.6693 & 0.8278 \\
Mask Consistency & 0.5444 & 0.2713 & 0.2576 & 0.8487 & 0.1760 & 0.5043 & 0.7904 & 0.9045 \\
Photometric Consistency & 0.4359 & 0.2632 & 0.2325 & 0.6427 & 0.1417 & 0.6097 & 0.8771 & 0.9494 \\
Pseudo Labelling & 0.4622 & 0.2503 & 0.2096 & 0.7200 & 0.1507 & 0.5853 & 0.8496 & 0.9368 \\
Vanilla T\textsuperscript{2}Net~\cite{t2net} & 0.4258 & 0.2532 & 0.2073 & 0.6372 & 0.1400 & 0.6183 & 0.8751 & 0.9496 \\
CrDoCo~\cite{chen2019crdoco} & 0.5459 & 0.2699 & 0.2550 & 0.8597 & 0.1752 & 0.5037 & 0.7910 & 0.9050 \\
Feature Consistency & 0.4766 & 0.2497 & 0.2181 & 0.7474 & 0.1582 & 0.5828 & 0.8321 & 0.9230 \\
Ground-Truth Training & 0.3062 & 0.1829 & 0.1178 & 0.4704 & 0.1052 & 0.7588 & 0.9307 & 0.9756 \\
Ours & 0.3375 & 0.1886 & 0.1266 & 0.5322 & 0.1125 & 0.7215 & 0.9218 & 0.9716
 \\
\bottomrule
\end{tabularx}
}
\caption{Online adaptation in speckle noise evaluated in the Stanford 2D-3D-S~\cite{stanford2d3d} dataset.}
\end{table*}

